Holistic Verification of Blockchain Consensus

Blockchain has recently attracted the attention of the industry due, in part, to its ability to automate asset transfers. It requires distributed participants to reach a consensus on a block despite the presence of malicious (a.k.a. Byzantine) participants. Malicious participants exploit regularly weaknesses of these blockchain consensus algorithms, with sometimes devastating consequences. In fact, these weaknesses are quite common and are well illustrated by the flaws in the hand-written proofs of existing blockchain consensus protocols [63]. Paradoxically, until now, no blockchain consensus has been holistically verified using model checking. In this paper, we remedy this paradox by model checking for the first time a blockchain consensus used in industry. We propose a holistic approach to verify the consensus algorithm of the Red Belly Blockchain [20], for any number $n$ of processes and any number $f<n/3$ of Byzantine processes. We decompose directly the algorithm pseudocode in two parts -- an inner broadcast algorithm and an outer decision algorithm -- each modelled as a threshold automaton [36], and we formalize their expected properties in linear-time temporal logic. We then automatically check the inner broadcasting algorithm, under a carefully identified fairness assumption. For the verification of the outer algorithm, we simplify the model of the inner algorithm by relying on its checked properties. Doing so, we formally verify not only the safety properties of the Red Belly Blockchain consensus but also its liveness in about 70 seconds.

==> alg/alg-bvb.tex <==

%\algnewcommand{\LeftComment}[1]{\Statex \(\triangleright\) #1}

\begin{algorithm}[t]
	\caption{The bv-broadcast algorithm at $p_i$\label{algo:bv-bcast}}
	{\footnotesize
	\begin{algorithmic}[1]
		\Part{$\lit{bv-broadcast}(\lit{MSG}, \ms{val}, i)$} { \Comment{binary value broadcast to filter out values proposed only by Byzantine processes} \label{line:bvbcast-start}
			\State $\lit{broadcast}(\lit{BV}, \ms{val}, i)$ \Comment{broadcast binary value $\ms{val}$} \label{line:bcast-1}
			\Repeat \Comment{re-broadcast a received value only if it is sufficiently represented}
				\If{$(\lit{BV}, \tup{v, *})$ received from $(t + 1)$ distinct processes 
				\State \T\T but not yet re-broadcast} \label{line:bcast-2}
					$\lit{broadcast}(\lit{BV}, v, i)$ \label{line:bvbcast-rebcast} 	
				\EndIf
				\If{$(\lit{BV}, \tup{v, *})$ received from $(2t + 1)$ distinct 
				\State \T\T processes}
					$\binvalues \leftarrow \binvalues \cup \{v\}$\label{line:BYZ-safe-14}\Comment{deliver $v$}%
				\EndIf%
			\EndRepeat \label{line:bvbcast-end}%
		}\EndPart%
	\end{algorithmic}%
	}
\end{algorithm}%

==> alg/alg-common-coin.tex <==
\begin{algorithm}[h!]
	\caption{The randomized consensus algorithm at $p_i$\label{alg:common-coin}}
	{\footnotesize
	\begin{algorithmic}[1]
	
%		\Part{{\bf State}}{
%			\State $\ms{val} \in \{0,1\}$, the estimate value, initially the input value
%			\State $r \in \mathbb{N}^*$, the round number, initially $1$
%			\State $\ms{contestants}, \ms{favorites}, \ms{qualifiers}$, three mappings from round numbers to sets of binary values, all indices mapping initially to $\emptyset$
%		}\EndPart
%		
%		\Statex
	
		\Part{$\lit{propose}(\ms{est})$} { \label{line:cc-binpropose}
%			\State $r \gets 0$ \label{line:cc-set-rnumber}
			\Repeat \label{line:cc-round-start} 
			\State $\BVbcast(\EST, \ms{est}, i) \to \binvalues$ \label{line:cc-BYZ-04} \Comment{binary value broadcast the current estimate} 
			\WUntil$(\binvalues \neq \emptyset$) \label{line:cc-BYZ-05}
				\Comment{wait enough time to receive some $\binvalues$}\EndWUntil
			\State $\lit{broadcast}(\AUX, \binvalues, i) \to \favorites$ \label{line:cc-BYZ-06} \Comment{broadcast second phase message}\label{line:cc-bincons:avcauxbcast}
			\WUntil $|\favorites| > n-t$	 and $\forall v \in \favorites, v \in \binvalues$	
				\EndWUntil \label{line:cc-BYZ-07} 
				\State $c \gets \lit{common-coin-toss}()$\label{line:cc-toss}
			\If{$\favorites = \{v\}$} \label{line:cc-BYZ-09} \Comment{if there is only one value, then adopt it}  \label{line:cc-BYZ-08}
				\State $\ms{est} \leftarrow v$  \Comment{estimate becomes this singleton value} \label{line:cc-BYZ-11}
				\If{$v = c$ and not decided yet}  $\lit{decide}(v)$ \label{line:cc-BYZ-10} \Comment{decide once if value matches parity} 
				\EndIf
				\Else{}
					 $\ms{est} \leftarrow c$   \Comment{otherwise, adopt the current parity bit} \label{line:cc-BYZ-12} 
			\EndIf
%			\State $r \leftarrow r + 1$; \label{line:inc-rnumber} \Comment{increment the round number}
			\EndRepeat \label{line:cc-round-end}
			%\Until{$\lit{decide}()$ was invoked in round $r-2$}\EndUntil  \label{line:stop}
		}\EndPart
		
		\end{algorithmic}
	}
\end{algorithm}

==> fig/bvb_ta.tex <==
\tikzstyle{node}=[circle,draw=black,thick,minimum size=4.3mm,inner sep=0.75mm,font=\normalsize]
\tikzstyle{init}=[node,fill=yellow!10]
\tikzstyle{final}=[node,fill=blue!10]
\tikzstyle{rule}=[->,thick]
\tikzstyle{post}=[->,thick,rounded corners,font=\normalsize]

\tikzset{every loop/.style={min distance=5mm,in=75,out=108,looseness=2}}


\begin{tikzpicture}[>=latex, thick, scale=0.85, every node/.style={scale=0.8},node distance=2cm]

% nodes

 \node at (0,0) [init,label=below:\textcolor{blue}{$V_0$}]    (V0) {};
 \node[below = 2cm of V0] [init,label=below:\textcolor{blue}{$V_1$}]   (V1) {};
 
 \node[right = 0.9cm of V0] [node,label=below:\textcolor{blue}{$B_0$}]   (B0) {}; 
 \node[right = 0.9cm of V1] [node,label=below:\textcolor{blue}{$B_1$}]   (B1) {};
 
 \node[right = 4cm of B0] [node,label=below:\textcolor{blue}{$CB_0$}]   (CB0) {}; 
 \node[right = 4cm of B1] [node,label=below:\textcolor{blue}{$CB_1$}]   (CB1) {};
 
 \node at ($(B0)!0.5!(CB1)$) [node,label=below:\textcolor{blue}{$B_{01}$}]   (B01) {}; 
 \node[above = of B01] [node,label=below:\textcolor{blue}{$C_{0}$}]   (C0) {};
 \node[below = of B01] [node,label=below:\textcolor{blue}{$C_1$}]   (C1) {};
  
 \node[right = 4cm of B01] [node,label=below:\textcolor{blue}{$C_{01}$}]   (C01) {}; 


% rules 


\draw[post] (V0) to[] 
	node[sloped, above, align=center] {$r_1\colon \cpp{b_0}$} (B0);
\draw[post] (V1) to[] 
	node[sloped, above, align=center] {$r_2\colon \cpp{b_1}$} (B1);

\draw[post] (B0) to[] 
	node[sloped, above, align=center] {$b_0 \ge 2t{+}1{-}f$} 
	node[sloped, below, align=center] {$r_3$} (C0);
\draw[post] (B0) to[] 
	node[sloped, above, align=center,pos=0.55] {$b_1{\ge}t{+}1{-}f \mapsto \cpp{b_1}$}
	node[sloped, below, align=center] {$r_4$} (B01);
\draw[post] (B1) to[] 
	node[sloped, above, align=center,pos=0.45] {$b_0{\ge}t{+}1{-}f \mapsto \cpp{b_0}$}
	node[sloped, below, align=center] {$r_5$} (B01);
\draw[post] (B1) to[] 
	node[sloped, above, align=center] {$b_1{\ge} 2t{+}1{-}f$} 
	node[sloped, below, align=center] {$r_6$}(C1);

\draw[post] (C0) to[] 
	node[sloped, above, align=center,pos=0.45] {$b_1{\ge}t{+}1{-}f \mapsto \cpp{b_1}$}
	node[sloped, below, align=center] {$r_7$} (CB0);
\draw[post] (B01) to[] 
	node[sloped, above, align=center] {$b_0 \ge 2t{+}1{-}f$}
	node[sloped, below, align=center] {$r_8$} (CB0);
\draw[post] (B01) to[] 
	node[sloped, above, align=center] {$b_1{\ge} 2t{+}1{-}f$} 
	node[sloped, below, align=center] {$r_{9}$}(CB1);
\draw[post] (C1) to[] 
	node[sloped, above, align=center,pos=0.45] {$b_0{\ge}t{+}1{-}f \mapsto \cpp{b_0}$}
	node[sloped, below, align=center] {$r_{10}$} (CB1);

\draw[post] (CB0) to[] 
	node[sloped, above, align=center] {$b_1{\ge} 2t{+}1{-}f$}
	node[sloped, below, align=center] {$r_{11}$} (C01);
\draw[post] (CB1) to[] 
	node[sloped, above, align=center] {$b_0 \ge 2t{+}1{-}f$}
	node[sloped, below, align=center] {$r_{12}$} (C01);




%self loops

\draw[rule,loop] (V0) to[] (V0);
\draw[rule,loop] (V1) to[] (V1);
%\draw[rule,loop] (B0) to[] (B0);
%\draw[rule,loop] (B1) to[] (B1);
%\draw[rule,loop] (B01) to[] (B01);
\draw[rule,loop] (C0) to[] (C0);
\draw[rule,loop] (C1) to[min distance=5mm,in=10,out=-23,looseness=2] (C1);
\draw[rule,loop] (CB0) to[] (CB0);
\draw[rule,loop] (CB1) to[min distance=5mm,in=10,out=-23,looseness=2] (CB1);
\draw[rule,loop] (C01) to[] (C01);

\end{tikzpicture}
